Identifying candidate routines for Robotic Process Automation from unsegmented UI logs

Robotic Process Automation (RPA) is a technology to develop software bots that automate repetitive sequences of interactions between users and software applications (a.k.a. routines). To take full advantage of this technology, organizations need to identify and to scope their routines. This is a challenging endeavor in large organizations, as routines are usually not concentrated in a handful of processes, but rather scattered across the process landscape. Accordingly, the identification of routines from User Interaction (UI) logs has received significant attention. Existing approaches to this problem assume that the UI log is segmented, meaning that it consists of traces of a task that is presupposed to contain one or more routines. However, a UI log usually takes the form of a single unsegmented sequence of events. This paper presents an approach to discover candidate routines from unsegmented UI logs in the presence of noise, i.e. events within or between routine instances that do not belong to any routine. The approach is implemented as an open-source tool and evaluated using synthetic and real-life UI logs.

==> algorithm1.tex <==
\begin{algorithm}[btp]
{
	\Input{Normalised UI log $\nuilog$}
	\Output{CFG  $(V,E,\hat{v},\hat{e})$}
	\BlankLine
	
	Set $V \leftarrow \varnothing$\;
	Set $E  \leftarrow \varnothing$\;

	create Map $\lambda : \bar{\Sigma} \rightarrow V$\;

	Vertex $\hat{v} \leftarrow$ new Vertex\;\label{alg:CFGinit1}
	Vertex $v_1 \leftarrow$ new Vertex\;
	add $v_1$ to $V$\;
	Normalised UI $\nui \leftarrow$ getUI($\nuilog$, $1$)\;
	$\lambda[\nui] \leftarrow v_1$\;
	Edge $\hat{e} \leftarrow (\hat{v},v_1)$\;\label{alg:CFGinit2}
		
	\BlankLine
	Vertex $v_2 \leftarrow$ null\;
	\For{ $i \in \left[ 2, \mathit{size}\left( \nuilog \right) \right]$}{
		
		$\nui \leftarrow$ getUI($\nuilog$, $i$)\;\label{alg:newvertex1}
		$v_2 \leftarrow \lambda[\nui]$\;\label{alg:newvertex11}
		\If{$v_2 = \mathit{null}$}{
				$v_2 \leftarrow$ new Vertex\;
				add $v_2$ to $V$\;
				$\lambda[\nui] \leftarrow v_2$\;
		}\label{alg:newvertex2}
			\lIf{$(v_1, v_2) \notin E$}{
				add $(v_1, v_2)$ to $E$\;\label{alg:newedge1}
			}
		$v_1 \leftarrow v_2$\;
	}
	\Return $(V,E,\hat{v},\hat{e})$
	\caption{Build CFG}\label{alg:buildCFG}
}
\end{algorithm}
\vspace{2mm}




==> algorithm5.tex <==
\begin{algorithm}[btp]
{
	\Input{Segments Set $\Psi$, Support Threshold $\mathit{minSup}$}
	\Output{Candidate Routines Set $R$}
	\BlankLine
	
	\Do{$P \neq \varnothing$}{
		$P \leftarrow$ findPatterns($\Psi$, $\mathit{minSup}$)\;
		$p \leftarrow$ selectBestPattern($P$)\;
		add $p$ to $R$\;
		removeOccurences($p$, $\Psi$)\;
	}

	\BlankLine
	\Return $R$\;
	
	\caption{Routine candidates identification}\label{alg:routineIdentification}
}
\end{algorithm}

==> authors_large.tex <==
\author{
\IEEEauthorblockN{Volodymyr Leno}
\IEEEauthorblockA{\textit{School of Computing and Information Systems} \\
\textit{University of Melbourne}\\
vleno@student.unimelb.edu.au}
\and
\IEEEauthorblockN{Adriano Augusto}
\IEEEauthorblockA{\textit{School of Computing and Information Systems} \\
\textit{University of Melbourne}\\
a.augusto@unimelb.edu.au}
\and
\IEEEauthorblockN{Marlon Dumas}
\IEEEauthorblockA{\textit{School of Computing and Information Systems} \\
\textit{University of Tartu}\\
marlon.dumas@ut.ee}
\and
\IEEEauthorblockN{Marcello La Rosa}
\IEEEauthorblockA{\textit{School of Computing and Information Systems} \\
\textit{University of Melbourne}\\
marcello.larosa@unimelb.edu.au}
\and
\IEEEauthorblockN{Artem Polyvyanyy}
\IEEEauthorblockA{\textit{School of Computing and Information Systems} \\
\textit{University of Melbourne}\\
artem.polyvyanyy@unimelb.edu.au}
\and
\IEEEauthorblockN{Luciano Garc\'ia-Ba\~nuelos}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
luciano@email.com}
}
